Screening Data Points in Empirical Risk Minimization via Ellipsoidal Regions and Safe Loss Functions

We design simple screening tests to automatically discard data samples in empirical risk minimization without losing optimization guarantees. We derive loss functions that produce dual objectives with a sparse solution. We also show how to regularize convex losses to ensure such a dual sparsity-inducing property, and propose a general method to design screening tests for classification or regression based on ellipsoidal approximations of the optimal set. In addition to producing computational gains, our approach also allows us to compress a dataset into a subset of representative points.

==> ellipsoid.tex <==
A subgradient of the \ref{s-lasso_pb} objective in $x$ is:
\begin{align*}
    A^t \ell'(Ax - b) + \lambda v_2
\end{align*}
with 
\begin{displaymath}
\ell'_i(u) \begin{cases}
            = 2 (u_i - \text{sgn}(u_i) \mu) & \text{if } |u_i| > \mu, \\
            = 0 & \text{otherwise}
            \end{cases}
            \end{displaymath}
and 
\begin{displaymath}
v_2^i(u) \begin{cases}
               = \text{sgn}(u_i) & \text{if } u_i \neq 0,\\
                \in [-1,1] & \text{otherwise}.
               \end{cases}
            \end{displaymath}

